Learning Ontologies with Epistemic Reasoning: The EL Case

We investigate the problem of learning description logic ontologies from entailments via queries, using epistemic reasoning. We introduce a new learning model consisting of epistemic membership and example queries and show that polynomial learnability in this model coincides with polynomial learnability in Angluin's exact learning model with membership and equivalence queries. We then instantiate our learning framework to EL and show some complexity results for an epistemic extension of EL where epistemic operators can be applied over the axioms. Finally, we transfer known results for EL ontologies and its fragments to our learning model based on epistemic reasoning.

==> monomial-EDL-decision.tex <==

To show Theorem~\ref{th:elk}, more work is needed.
%
A first approach might be to adapt the tableaus for $S5_n$ from~\cite{HALPERN1992319} to the case of \ELK.
%
When applied to monomial \ELK formulas, it is not difficult to see that in the tableau procedure the OR-rule is not a cause of inefficiency any more. Roughly speaking, this is because with monomial \ELK formulas, the OR-rule would be the last rules applied in a branch.
%
However, the procedure would still yield an exponential time decision procedure.
%
The main problem resides in the full expansions of propositional tableaus, because it causes a branching for every subformula not yet determined in a node.
%

For this reason, we propose an ad-hoc decision procedure to decide the satisfiability of $\ELK$ formulas restricted to monomials. It is presented as Algorithm~\ref{A:monomial-elk-sat}.

\medskip

We will need some additional notation.
For every $\sigma = a_1 \ldots a_k \in \agents^*$ we note $\Rmc_\sigma = \Rmc_{a_1} \circ \ldots \circ \Rmc_{a_k}$ and $\KK_\sigma = \K_{a_1} \ldots \K_{a_k}$.
The empty series is noted $\epsilon$, and we have $\Rmc_\epsilon = Id$ and $\KK_\epsilon \omega = \omega$.
We simply note $\beta \in \psi$ to indicate that $\beta$ is a conjunct occurring in $\psi$.

Let $\sigma$ and $\sigma'$ be two series of agents. We say that $\sigma'$ is a \emph{subword} of $\sigma$ when $\sigma'$ is the result of removing zero or more elements from $\sigma$.


Let $\varphi_0$ be a monomial $\ELK$ formula. That is, $\varphi_0$ is of the form:
\[
\begin{array}{cc}
  \omega_0 & \land\\
  \KK_{\sigma_1} \omega_{\sigma_1} \land \ldots \land \KK_{\sigma_n} \omega_{\sigma_n} & \land\\  
  \lnot \KK_{\sigma_{n+1}} \omega_{\sigma_{n+1}} \land \ldots \land \lnot \KK_{\sigma_m} \omega_{\sigma_m} &\\
\end{array}
\]
where $\sigma_i \in \agents^+$, for every $1 \leq i \leq m$, is a non-empty series of agents.
and, each $\omega_i$ with $0 \leq i \leq m$, is a conjunction of literals of \EL axioms.
We note $\varphi^\flat_0$ the formula resulting from substituting every immediate repetitions $a \ldots a$ of an agent $a$ occurring in $\sigma_i$, $1 \leq i \leq m$, with $a$.

\begin{algorithm}
\caption{$SAT(\varphi_0)$, deciding the satisfiability of monomial \ELK formulas\label{A:monomial-elk-sat}}
\begin{algorithmic}[1]
\Require A monomial \ELK formula $\varphi_0$
\Ensure TRUE if $\varphi_0$ is satisfiable, and FALSE otherwise
\State $\varphi^\flat_0 = \omega_0 \land
  \KK_{\sigma_1} \omega_{\sigma_1} \land \ldots \land \KK_{\sigma_n} \omega_{\sigma_n} \land  
  \lnot \KK_{\sigma_{n+1}} \omega_{\sigma_{n+1}} \land \ldots \land \lnot \KK_{\sigma_m} \omega_{\sigma_m}$
\If {$\omega_0 \land \bigwedge \{ \omega \mid \KK_\sigma \omega \in \varphi^\flat_0 \}$ is not \EL consistent}
\State \Return{FALSE}
\EndIf
\For {$\lnot \KK_{\sigma}\omega \in \varphi^\flat_0$}
\State \label{lab:algo-start-check} $\psi = \top \land \bigwedge \{ \omega' \mid \KK_{\sigma'} \omega' \in \varphi^\flat_0, \text{ and } \sigma \text{ is a subword of } \sigma' \}$
\State $MS = \{\psi \land \lnot \beta \mid \beta \text{ is an \EL literal in }  \omega \}$
\If{all \EL monomials in $MS$ are not \EL consistent} 
\State \Return {FALSE}
\EndIf \label{lab:algo-end-check}
\EndFor
\State \Return {TRUE}
\end{algorithmic}
\end{algorithm}

\medskip

The two following lemmas are simple consequences of well-known properties of the modal system $S5$~\cite[p.~58]{HughesCresswell}.
\begin{lemma}\label{lem:flat-equiv}
  If $\varphi^\flat_0$ is an \ELK formula,
$\varphi_0$ and $\varphi^\flat_0$ are equivalent.
\end{lemma}
\begin{proof}
  For every $i \in \agents$, $\Rmc_i$ is an equivalence relation. In particular it is transitive and reflexive, and we have $\Rmc_i\circ \Rmc_i = \Rmc_i$. Thus, for every pointed interpretation $(\Imf,\Imc)$, for every agent $i \in \agents$, and for every formula $\varphi$, we have $(\Imf,\Imc) \models \K_i\K_i\varphi$ iff $(\Imf,\Imc) \models \K_i\varphi$.
\end{proof}

\begin{lemma}\label{lem:subword}
Let $\sigma$ and $\sigma'$ be two series of agents in $\agents^*$.
If $\sigma$ is a subword of $\sigma'$ then $\Rmc_{\sigma} \subseteq \Rmc_{\sigma'}$.
\end{lemma}
\begin{proof}
  For every $i \in \agents$, because $\Rmc_i$ is an equivalence relation, and thus reflexive, we have $Id \subseteq \Rmc_i$. We can thus insert arbitrarily additional agents in the occurence of $\sigma$ appearing
  in the right-hand side of $\Rmc_{\sigma} \subseteq \Rmc_{\sigma}$, and obtain the result.
\end{proof}

The following proposition is central to the correctness of Algorithm~\ref{A:monomial-elk-sat}.
\begin{proposition}\label{prop:corr-monom-EL}
Let $\varphi_0$ be the monomial \ELK formula, such that $\varphi^\flat_0$ is of the form \[\omega_0 \land
  \KK_{\sigma_1} \omega_{\sigma_1} \land \ldots \land \KK_{\sigma_n} \omega_{\sigma_n} \land  
  \lnot \KK_{\sigma_{n+1}} \omega_{\sigma_{n+1}} \land \ldots \land \lnot \KK_{\sigma_m} \omega_{\sigma_m}
  \enspace .\] $\varphi_0$ is unsatisfiable iff at least one of the following properties holds:
  \begin{enumerate}
  \item $\omega_0 \land \bigwedge \{ \omega \mid \KK_{\sigma} \omega \in \varphi^\flat_0 \}$ is not \EL consistent;
  \item there is $\lnot \KK_{\sigma}\omega \in \varphi^\flat_0$ such that $\lnot\omega \land \bigwedge \{ \omega' \mid \KK_{\sigma'}\omega' \in \varphi^\flat_0, \text{ and } \sigma \text{ is a subword of } \sigma' \}$ is not \EL consistent.
  \end{enumerate}
\end{proposition}
\begin{proof}
Since by Lemma~\ref{lem:flat-equiv}, $\varphi^\flat_0$ and $\varphi_0$ are equisatisfiable, we prove the property for $\varphi^\flat_0$.

Right to left. Suppose (1) holds. Since $\Rmc_i$ is reflexive for all $i \in \agents$, every model satisfying $\varphi^\flat_0$ must satisfy $\omega_0 \land \bigwedge \{ \omega \mid \KK_{\sigma} \omega \in \varphi^\flat_0 \}$. Since it is not \EL satisfiable, there cannot be an \ELK interpretation satisfying $\varphi^\flat_0$ either. Suppose (2) holds. For some $\lnot \KK_{\sigma}\omega \in \varphi^\flat_0$, we have that $\varphi = \lnot\omega \land \bigwedge \{ \omega' \mid \KK_{\sigma'}\omega' \in \varphi^\flat_0, \text{ and } \sigma \text{ is a subword of } \sigma' \}$ is not \EL consistent.
%
Suppose towards contradiction that there exist
an \ELK interpretation $\Imf=(\Wmc,\{\Rmc_i\}_{i\in \agents})$ and an \EL interpretation $\Jmc \in \Wmc$ such that $(\Imf, \Jmc) \models \varphi^\flat_0$. It means that 
$(\Imf, \Jmc) \models \lnot \KK_{\sigma}\omega$, that is, there is an \EL interpretation $\Jmc$ such that $(\Jmc, \Jmc') \in \Rmc_\sigma$ and $(\Imf, \Jmc') \models \lnot \omega$.
%
From Lemma~\ref{lem:subword}, for every $\KK_{\sigma'}\omega' \in \varphi^\flat_0$, if $\sigma$ is a subword of $\sigma'$, then $\Rmc_{\sigma} \subseteq \Rmc_{\sigma'}$. Hence, it must be the case that $(\Imf, \Jmc') \models \varphi$; a contradiction because $\varphi$ is not \EL consistent.


Left to right. Assume that none of (1) and (2), we must show that $\varphi^\flat_0$ is satisfiable.
It suffices to build an \ELK interpretation $\Imf=(\Wmc,\{\Rmc_i\}_{i\in \agents})$ for $\varphi^\flat_0$, such that:
\begin{itemize}
\item Construction of $\Wmc$. $\Wmc$ contains an \EL interpretation $\Jmc_0$ satisfying $\omega_0 \land \bigwedge \{ \omega \mid \KK_{\sigma} \omega \in \varphi^\flat_0 \}$. Such an interpretation exists because (1) does not hold.
%
For each $\lnot \KK_{\sigma}\omega \in \varphi^\flat_0$, where $\sigma = a_1 \ldots a_k$, $\Wmc$ also contains an interpretation $\Jmc^\sigma_k$ satisfying
$\lnot\omega \land \bigwedge \{ \omega' \mid \KK_{\sigma'}\omega' \in \varphi^\flat_0, \text{ and } \sigma \text{ is a subword of } \sigma' \}$.
Such an interpretation exists because (2) does not hold.
%
Still for each $\lnot \KK_{\sigma}\omega \in \varphi^\flat_0$, $\Wmc$, where $\sigma = a_1\ \ldots a_k$, for each $1 \leq i < k$,
$\Wmc$ also contains an interpretation $\Jmc^\sigma_i$ satisfying
$\bigwedge \{ \omega' \mid \KK_{\sigma'}\omega' \in \varphi^\flat_0, \text{ and } a_1 \ldots a_i \text{ is a subword of } \sigma' \}$. Such interpretations exist because (1) does not hold.
%
$\Wmc$ does not contain any more \EL interpretations.
\item Construction of $\Rmc$. For every $\lnot \KK_{\sigma}\omega \in \varphi^\flat_0$, where $\sigma = a_1 \ldots a_k$, for every $1 \leq i \leq k$, let $(\Jmc^\sigma_{i-1}, \Jmc^\sigma_i) \in \Rmc'_{a_i}$, where $\Jmc^\sigma_{0} = \Jmc_{0}$. For every $i \in \agents$, let $\Rmc_i$ be the equivalence closure of $\Rmc'_i$.
\end{itemize}
It is routine to check that $\Imf, \Jmc_0 \models \varphi^\flat_0$.
\end{proof}

\medskip

Proposition~\ref{prop:corr-monom-EL} suggests that the satisfiability of monomial \EL formulas can be reduced to checking the consistency of conjunctions of \EL literals. Reasoning about the consistency of conjunctions of \EL literals can be delegated to the reasoning in \ELPP~\cite{BBL-EL}.
We define the function $\tau$ from the set of \EL literals to the set of subsets of \ELPP CBox axioms as follows:
\[
\begin{array}{lcl}
\tau(A(a)) &  := & \{ \{a\} \sqsubseteq A \}\\
\tau(\lnot A(a)) &  := & \{ \{a\} \sqcap A \sqsubseteq \bot \}\\
\tau(C \sqsubseteq D) &  := &  \{ C \sqsubseteq D \}\\
\tau(\lnot (C \sqsubseteq D)) &  := &  \{ \{f\} \sqsubseteq C , \{f\} \sqcap D \sqsubseteq \bot \} \hfill , \text{where $f$ is a fresh individual} \\
\tau(r(a,b)) &  := &  \{ \{a\} \sqsubseteq \exists r. \{b\} \}\\
\tau(\lnot r(a,b)) &  := &   \{ \{a\} \sqcap \exists r. \{b\} \sqsubseteq \bot \}
\end{array}
\]
Now, with \elaxiomlit an \EL axiom literal and $L$ a set of \EL axiom literals, define:
\[
\begin{array}{lcl}
  \tau^\bullet(\emptyset) & := & \emptyset\\
  \tau^\bullet(\{ \elaxiomlit \} \cup L) & := &  \tau(\elaxiomlit) \cup \tau^\bullet(L)
\end{array}
\]
The semantics of the new syntax are: $(\{a\})^\Imc =  \{a^\Imc\}$ and $(\bot)^\Imc = \emptyset$.


An analogous reduction is presented in the proof of~\cite[Lemma~2.1]{Thost2015LTLOE}.
It is routine to show the next proposition.
\begin{proposition}\label{prop:elpp-onto-compl}
The set of \EL axiom literals $L$ is consistent iff $\tau^\bullet(L)$ is a consistent \ELPP ontology.
\end{proposition}

\medskip

We are finally ready to prove the complexity of deciding whether a monomial \ELK formula is satisfiable.

\TheoremConjunction*

%% \begin{proposition}
%% The problem of checking whether a monomial \ELK formula $\varphi_0$ is satisfiable is in PTIME.
%% \end{proposition}
\begin{proof}
%  The problem of checking whether a monomial \ELK formula $\varphi_0$ is satisfiable is in \PTime.
%
  Consider Algorithm~\ref{A:monomial-elk-sat}. The monomial \ELK formula $\varphi_0$ is satisfiable iff $SAT(\varphi_0)$ returns TRUE. The correctness of the algorithm follows immediately from Prop.~\ref{prop:corr-monom-EL}. It suffices to observe that items~\ref{lab:algo-start-check}--\ref{lab:algo-end-check} check the inconsistency of an \EL formula $\lnot\omega \land \psi$ where $\omega$ is a conjunction of \EL literals and $\psi$ is a monomial \EL formula (observe that $\lnot\omega \land \psi$ is not a monomial \EL formula, unless $\omega$ contains only one literal) by checking the inconsistency of as many monomial \EL formulas $\lnot \beta \land \psi$ as there are literals $\beta$ in $\omega$.
%
A simple analysis shows that the algorithm runs in time polynomial in the size of $\varphi_0$, with a polynomial number of calls to a procedure for checking the inconsistency of conjunctions of \EL literals. From Prop.~\ref{prop:elpp-onto-compl} and \cite{BBL-EL} we know that each of these checks can be done in polynomial time. Membership in \PTime follows.
\end{proof}



==> relatedwork.tex <==
%Regarding combinations of \EL and epistemic logic 
%We point out an  



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

